MeetUp! A Corpus of Joint Activity Dialogues in a Visual Environment

Building computer systems that can converse about their visual environment is one of the oldest concerns of research in Artificial Intelligence and Computational Linguistics (see, for example, Winograd's 1972 SHRDLU system). Only recently, however, have methods from computer vision and natural language processing become powerful enough to make this vision seem more attainable. Pushed especially by developments in computer vision, many data sets and collection environments have recently been published that bring together verbal interaction and visual processing. Here, we argue that these datasets tend to oversimplify the dialogue part, and we propose a task---MeetUp!---that requires both visual and conversational grounding, and that makes stronger demands on representations of the discourse. MeetUp! is a two-player coordination game where players move in a visual environment, with the objective of finding each other. To do so, they must talk about what they see, and achieve mutual understanding. We describe a data collection and show that the resulting dialogues indeed exhibit the dialogue phenomena of interest, while also challenging the language & vision aspect.

==> figures/dial1.tex <==
\begin{tabular}{lrl}
\toprule
{} &     time &                                                                                                                                                                                                                                                main \\
\midrule
10 & 00:03 &  \emph{GM (to A): url: /b/bathroom/ADE-train-00002739.jpg} \\
12 & 00:03 &  \emph{GM (to A): You can go: [/s]outh [/n]orth [/w]est} \\
14 & 00:03 &  \emph{GM (to A): You have to meet in: b/basement} \\
15 & 00:03 &  \emph{GM (to B): url: /a/apartment-building/outdoor/ADE-train-00001414.jpg} \\
17 & 00:04 &  \emph{GM (to B): You can go: [/s]outh} \\
19 & 00:04 &  \emph{GM (to B): You have to meet in: b/basement} \\
20 & 00:18 &  \textbf{A: i am in the bathroom} \\
21 & 00:29 &  \textbf{A: where are you at?} \\
22 & 00:33 &  \textbf{B: I'm outside. Let's move around a bit.} \\
23 & 00:38 &  \textbf{A: k} \\
24 & 00:40 &  B (privately): n \\
25 & 00:41 &  \emph{GM (to B): Nothing happened.You can go: [/s]outh} \\
26 & 00:43 &  A (privately): s \\
27 & 00:44 &  \emph{GM (to A): url: /b/bedroom/ADE-train-00003553.jpg} \\
29 & 00:44 &  \emph{GM (to A): You can go: [/s]outh [/n]orth [/w]est} \\
30 & 00:45 &  B (privately): s \\
31 & 00:45 &  \emph{GM (to B): url: /b/basement/ADE-train-00002497.jpg} \\
33 & 00:45 &  \emph{GM (to B): You can go: [/s]outh [/n]orth [/e]ast} \\
34 & 00:50 &  A (privately): s \\
35 & 00:50 &  \emph{GM (to A): url: /c/corridor/ADE-train-00006285.jpg} \\
37 & 00:51 &  \emph{GM (to A): You can go: [/n]orth [/e]ast} \\
38 & 00:52 &  B (privately): s \\
39 & 00:52 &  \emph{GM (to B): url: /l/living-room/ADE-train-00000774.jpg} \\
41 & 00:53 &  \emph{GM (to B): You can go: [/s]outh [/n]orth [/e]ast} \\
42 & 00:57 &  B (privately): s \\
43 & 00:57 &  \emph{GM (to B): url: /b/basement/ADE-train-00002482.jpg} \\
45 & 00:57 &  \emph{GM (to B): You can go: [/n]orth [/e]ast} \\
46 & 01:01 &  A (privately): e \\
47 & 01:01 &  \emph{GM (to A): url: /b/basement/ADE-train-00002494.jpg} \\
49 & 01:01 &  \emph{GM (to A): You can go: [/e]ast [/w]est} \\
50 & 01:11 &  \textbf{A: I am in the basement} \\
51 & 01:11 &  \textbf{B: I'm in a basement.} \\
52 & 01:23 &  \textbf{B: Mine has a white staircase} \\
53 & 01:28 &  \textbf{A: no} \\
54 & 01:37 &  \textbf{A: mine has wooden stair case} \\
55 & 01:55 &  \textbf{B: Okay. Should I try to move towards you?} \\
56 & 02:09 &  \textbf{A: Sure} \\
57 & 02:11 &  \textbf{B: Wooden? What else?} \\
58 & 02:16 &  B (privately): e \\
59 & 02:17 &  \emph{GM (to B): url: /b/bedroom/ADE-train-00003553.jpg} \\
61 & 02:17 &  \emph{GM (to B): You can go: [/s]outh [/n]orth [/w]est} \\
62 & 02:25 &  B (privately): s \\
63 & 02:25 &  \emph{GM (to B): url: /c/corridor/ADE-train-00006285.jpg} \\
65 & 02:25 &  \emph{GM (to B): You can go: [/n]orth [/e]ast} \\
66 & 02:27 &  \textbf{A: water heater and washer and dryer} \\
67 & 02:35 &  B (privately): s \\
68 & 02:35 &  \emph{GM (to B): Nothing happened.You can go: [/n]orth [/e]ast} \\
69 & 02:40 &  B (privately): e \\
70 & 02:40 &  \emph{GM (to B): url: /b/basement/ADE-train-00002494.jpg} \\
72 & 02:41 &  \emph{GM (to B): You can go: [/e]ast [/w]est} \\
73 & 02:42 &  \textbf{A: a plastic chair and a screen door} \\
74 & 03:01 &  \emph{GM: Attention: you are in the game for 3 minutes!} \\
75 & 03:18 &  \textbf{B: I'm there! I see the water heater, washer and dryer, sink, chair laying on top of the screen door} \\
76 & 03:26 &  B (privately): done \\
77 & 03:27 &  \emph{GM: The '/done' command has been issued                                        by you or your partner.                                        To end the game, both players                                        need to enter '/done'} \\
78 & 03:27 &  \textbf{A: yep} \\
79 & 03:32 &  A (privately): done \\
80 & 03:34 &  \emph{GM: Well done! Both of you are                            indeed in the same room of type: b/basement!} \\
\bottomrule
\end{tabular}




==> figures/dial2.tex <==
\begin{tabular}{lrl}
\toprule
{} &     time &                                                                                    main \\
\midrule
80 & 00:42 &  \textbf{A: i think i am in a basement} \\
81 & 00:48 &  \textbf{B: i think i might be too.} \\
82 & 00:52 &  \textbf{A: maybe not though} \\
83 & 01:00 &  \textbf{A: wood panel?} \\
84 & 01:04 &  \textbf{A: two doors?} \\
85 & 01:07 &  \textbf{B: there's a tan couch, and a tan loveseat/chair. brown coffee table. bar. tv} \\
86 & 01:10 &  \textbf{B: nope, different room} \\
87 & 01:13 &  \textbf{A: ok i am not there} \\
88 & 01:23 &  \textbf{B: want me to meet you, or do you want to meet me?} \\
89 & 01:34 &  \textbf{A: i think mine is more basement like} \\
90 & 01:39 &  \textbf{B: okay. i'll try to find it.} \\
\bottomrule
\end{tabular}

